Filling Gender & Number Gaps in Neural Machine Translation with Black-box Context Injection

When translating from a language that does not morphologically mark information such as gender and number into a language that does, translation systems must "guess" this missing information, often leading to incorrect translations in the given context. We propose a black-box approach for injecting the missing information to a pre-trained neural machine translation system, allowing to control the morphological variations in the generated translations without changing the underlying model or training data. We evaluate our method on an English to Hebrew translation task, and show that it is effective in injecting the gender and number information and that supplying the correct information improves the translation accuracy in up to 2.3 BLEU on a female-speaker test set for a state-of-the-art online black-box system. Finally, we perform a fine-grained syntactic analysis of the generated translations that shows the effectiveness of our method.

==> Filling Gender & Number Gaps (short)/resources/french.tex <==
\begin{table}[h]
\begin{center}
    
\begin{tabular}{|l|l|l|}
\hline
                                     & Male  & Female \\ \hline
VHW \citeyearpar{vanmassenhove-hardmeier-way:2018:EMNLP} Baseline & 37.58 & 37.75  \\ \hline
VHW \citeyearpar{vanmassenhove-hardmeier-way:2018:EMNLP} + TAG    & 38.71 & 38.97  \\ \hline
Google Translate                     & 39.33 & 39.02  \\ \hline
Google Translate + Prefix            & 39.95 & 39.95  \\ \hline
\end{tabular}
\caption{Comparison of our approach (using Google Translate) to \citet{vanmassenhove-hardmeier-way:2018:EMNLP} on their English-French gender corpus.}
\label{table:french}

\end{center}
\end{table}

==> Filling Gender & Number Gaps (short)/resources/going-to-kill-you.tex <==
\begin{table*}
	\centering
	\begin{tabular}{|l|l|l|l|}
		\hline
		\textbf{Prefix}                & \textbf{Speaker}                                      & \textbf{Interlocutor Gender}                         & \textbf{Interlocutor Number}                          \\ \hline
		He said to him        & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		He said to her        & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{FE0000} \xmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		He said to them       & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		He said to the girls  & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{FE0000} \xmark} & {\color[HTML]{FE0000} \xmark} \\ \hline
		She said to him       & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		She said to her       & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{FE0000} \xmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		She said to them      & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		She said to the girls & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{FE0000} \xmark} & {\color[HTML]{FE0000} \xmark} \\ \hline
	\end{tabular}
	\caption{Does feeding information to Google Translate successfully change dependent words?}
	\label{table:going-to-kill-you}
\end{table*}

==> Filling Gender & Number Gaps (short)/resources/languages.tex <==
\newcommand\good[1]{{\color[HTML]{32cb00} #1}}
\newcommand\bad[1]{{\color[HTML]{FD6864} #1}} 


\begin{table*}[t]
	\centering
\begin{tabular}{|l|l|l|l|}
\hline
           & English Text          & Masculine                                    & Feminine                                     \\ \hline
Hebrew     & I am nice             & ani nehmad                                   & ani nehmada                                  \\ \hline
\multicolumn{2}{|l|}{Prefix}       & ani \good{nehmad}           & ani \good{nehmada}          \\ \hline
Spanish    & I am delighted        & Estoy encantado                              & Estoy encantada                              \\ \hline
\multicolumn{2}{|l|}{Prefix}       & Estoy \good{encantado}      & Estoy \good{encantada}      \\ \hline
Portuguese & I was called          & Eu fui chamado                               & Eu fui chamada                               \\ \hline
\multicolumn{2}{|l|}{Prefix}       & Eu fui \good{chamado}       & Eu fui \bad{chamado}       \\ \hline
French     & I am patient          & je suis patient                              & je suis patiente                             \\ \hline
\multicolumn{2}{|l|}{Prefix}       & je suis \good{patient}      & je suis \good{patiente}     \\ \hline
Italian    & I am beautiful        & Sono bello                                   & Sono bella                                   \\ \hline
\multicolumn{2}{|l|}{Prefix}       & io sono \good{bello}        & io sono \good{bella}        \\ \hline
Russian    & I wrote a message     & \foreignlanguage{russian}{Я написал сообщение}& \foreignlanguage{russian}{Я написала сообщение} \\ \hline
\multicolumn{2}{|l|}{Prefix}       & \foreignlanguage{russian}{Я \good{написал} сообщение}  & \foreignlanguage{russian}{Я \bad{написал} сообщение}  \\ \hline
Czech      & I gave her the flower & já jsem ji dal květinu                       & já jsem ji dala květinu                      \\ \hline
\multicolumn{2}{|l|}{Prefix}       & \bad{Dala} jsem jí květinu & \good{Dala} jsem jí květinu \\ \hline
Romanian   & I am patient          & Sunt răbdător                                & Sunt răbdătoare                              \\ \hline
\multicolumn{2}{|l|}{Prefix}       & Sunt \good{răbdător}        & Sunt \good{răbdătoare}      \\ \hline
Catalan    & I am rich             & sóc ric                                      & sóc rica                                     \\ \hline
\multicolumn{2}{|l|}{Prefix}       & sóc \good{ric}              & sóc \bad{ric}              \\ \hline
Polish     & I am nice             & Jestem miły                                  & Jestem miła                                  \\ \hline
\multicolumn{2}{|l|}{Prefix}       & Jestem \good{miły}          & Jestem \good{miła}          \\ \hline
\end{tabular}
\caption{Examples of languages where the speaker's gender changes morphological markings in different languages, and translations using the prefix ``He said:'' or ``She said:'' accordingly}
\label{table:languages}
\end{table*}

==> Filling Gender & Number Gaps (short)/results/silverman.tex <==
% \centering
%             \begin{tabular}{|l|l|l|l|l|l|l|}
%             \hline
%              Gender & Audience & BLEU & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 \\
%              \Xhline{2\arrayrulewidth}

%             She & her   &       20.98   &52.7&26.6&15.4&9.0 \\ \hline 
%             She & them  &       20.97   &52.7&26.6&15.4&9.0 \\ \hline 
%             She & him   &       20.82   &52.5&26.3&15.1&9.0 \\ \hline 
%             She &       &       20.8    &52.5&26.4&15.2&8.9 \\ \hline 
%             I   & them  &       20.23   &52.5&26.0&14.6&8.4 \\ \hline 
%             I   &       &       19.84   &51.8&25.2&14.2&8.4 \\ \hline 
%             He  & them  &       19.5    &51.8&25.2&13.9&8.0 \\ \hline 
%             He  & her   &       19.3    3&51.7&24.9&13.7&7.9 \\ \hline 
%             He  & him   &       19.25   &51.4&24.7&13.7&7.9 \\ \hline 
%             He  &       &       19.2    &51.0&24.5&13.7&8.0 \\ \Xhline{2\arrayrulewidth}
% \multicolumn{2}{|c|}{Baseline}& 18.67   &49.9&23.8&13.3&7.7
%             \\ \hline
%             \end{tabular}
%             \caption{BLEU results with a single reference}
%             \label{table:results-silverman}

\centering
\begin{tabular}{|l|l|l|}
\hline
Speaker & Audience & BLEU \\
\Xhline{2\arrayrulewidth}
\multicolumn{2}{|c|}{Baseline}& 18.67 \\ \Xhline{2\arrayrulewidth}

He  & --    &       19.2    \\ \hline
He  & him   &       19.25   \\ \hline 
He  & her   &       19.3    \\ \hline 
He  & them  &       19.5    \\ \hline
I   & --    &       19.84   \\ \hline 
I   & them  &       20.23   \\ \hline 
She & --    &       20.8    \\ \hline 
She & him   &       20.82   \\ \hline 
She & her   &       20.98   \\ \hline
She & them  &       20.97   \\ \hline 

            \end{tabular}
            \caption{BLEU results on the Silverman dataset}
            % \am{Any reason not to sort this?}
            \label{table:results-silverman}
            

==> resources/going-to-kill-you.tex <==
\begin{table*}
	\centering
	\begin{tabular}{|l|l|l|l|}
		\hline
		\textbf{Prefix}                & \textbf{Speaker}                                      & \textbf{Interlocutor Gender}                         & \textbf{Interlocutor Number}                          \\ \hline
		He said to him        & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		He said to her        & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{FE0000} \xmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		He said to them       & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		He said to the girls  & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{FE0000} \xmark} & {\color[HTML]{FE0000} \xmark} \\ \hline
		She said to him       & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		She said to her       & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{FE0000} \xmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		She said to them      & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{32CB00} \cmark} \\ \hline
		She said to the girls & {\color[HTML]{32CB00} \cmark} & {\color[HTML]{FE0000} \xmark} & {\color[HTML]{FE0000} \xmark} \\ \hline
	\end{tabular}
	\caption{Does feeding information to Google Translate successfully change dependent words?}
	\label{table:going-to-kill-you}
\end{table*}
